Renormalization and existence of the finite-time blow up solutions for a one-dimensional analogue of the Navier-Stokes equations

The one-dimensional quasi-geostrophic equation is the one-dimensional Fourier-space analogue of the famous Navier-Stokes equations. In their work Li and Sinai have proposed a renormalization approach to the problem of existence of finite-time blow up solutions of this equation. In this setting, existence of finite time blow ups is a consequence of existence of a fixed point for a certain renormalization operator on an appropriate functional space. They have provided a proof of existence of complex-valued finite time blow up solutions of the quasi-geostrophic equation. In this paper we revisit the renormalization problem for the quasi-geostrophic blow ups, prove existence of a family of renormalization fixed points, and deduce existence of real $C^\infty([0,T),C^\infty(\mathbb{R}) \cap L^2(\mathbb{R}))$ solutions to the quasi-geostrophic equation whose energy and enstrophy become unbounded in finite time, different from those found in the previous work of Li and Sinai.

==> prelims.tex <==
\section{Introduction}
  
We start with a brief review of the models that has been considered in the literature.

\subsection{The Navier-Stokes equations}

Recall the famous Navier-Stokes equations
\begin{equation}\label{eq:NS}
\partial_t u + (u \cdot \nabla) u - \nu \Delta u + \nabla p = g\,, 
\qquad
\nabla \cdot u =0\,, 
\qquad
u(\cdot,0)=u_0
\end{equation}
where 
$g : \RR^d \times \RR \rightarrow \RR^d$ 
is an external force, and $u_0: \RR^d \rightarrow \RR^d$ is the initial datum. The unknowns are
$u : \RR^d \times \RR \rightarrow \RR^d$ and $p : \RR^d \times \RR \rightarrow \RR$.
We set the viscosity $\nu=1$, and we are interested in $d \geq 3$
and $g \equiv 0$.

%We apply Fourier transform \footnote{The notation $y$ for the frequency space seems more standard (e.g. Evans) The use of $k$ is more typical in the periodic case (i.e. $\TT^d$ rather than $\RR^d$) since it belongs to a discrete set.} $v(y)=\cF[u](y)$, given by
We apply the Fourier transform  $v(y)=\cF[u](y)$, given by

\[
v(y,t)=\int_{\RR^d} u(x,t) \ee^{-\ii y \cdot x} \dif x\,,
\qquad
u(x,t)=\int_{\RR^d} v(y,t) \ee^{\ii y \cdot x} \dif y\,,
\]
so that the Navier-Stokes PDE becomes the following system of integro-differential equations:
\begin{equation}\label{eq:sist:FT}
\frac{\pd v(y,t)}{\pd t} = -|y|^2 v(y,t) + \ii \int_{\RR^d} (y \cdot v(y-z,t)) P_y v(z,t) \dif z \,,
\qquad
\end{equation}
where $P_y$ is the {\it Leray} orthogonal projection to the subspace orthogonal to $y$, i.e.
\begin{equation}\label{eq:leray}
P_y v = v - \frac{v \cdot y}{|y|^2} y\,.
\end{equation}

\begin{remark}
The incompressibility condition $\nabla \cdot u=0$ reads $v(y,t) \cdot y =0$ in
Fourier space. % We observe that $P_y v(y,t)=v(y,t)$.
\end{remark}

\begin{remark}
If $u : \RR^d \times \RR \rightarrow \RR$ then $v:\RR^d\times \RR \rightarrow \CC$
satisfies the symmetry property
\[
v(y,t)=\overline{v(-y,t)}\,,\qquad \forall t \in \RR\,.
\]
%This condition is useful to save memory and computations, ensuring that we obtain real solution for NS. For example, we only need to store the values of $v$ in $\RR^{d-1} \times \RR_+$.
\end{remark}

Integrating \eqref{eq:sist:FT} with respect to $t$, we obtain the integral equations:
\begin{equation}\label{eq:integral:NS}
v(y,t) = \ee^{-|y|^2 t} v_0(y) + \ii \int_0^t \int_{\RR^d} (y \cdot v(y-z,\tau)) P_y v(z,\tau)
\ee^{-|y|^2 (t-\tau)} \dif z \dif \tau\,,
\end{equation}
where $v_0=v(y,0)$ stands for the initial datum at $t=0$.


\subsection{The quasi-geostrophic equation}
Our primary focus will be  equation $(\ref{eq:modelB})$, which according to the discussion of \cite{CCCF} is a one-dimensional version of the 2D quasi-geostrophic initial value problem:
\begin{eqnarray} 
\label{QC1} &&\theta_t + (u \cdot \nabla) \theta=0, \\
\label{QC2}  && u=\nabla^{\perp} \psi, \quad \nabla^{\perp} := (-\partial_2, \partial_1), \\
\label{QC3}  && \theta=-(-\Delta)^{1 \over 2} \psi, \\
\label{QC4}  && \theta(x,0)=\theta_0(x).
\end{eqnarray}
This system of equations models the evolution of the temperature in a mixture of cold and hot air fronts. Equations $(\ref{QC2})-(\ref{QC3})$ can be written as
$$u= - R^{\perp} \theta=-(R_2 \theta, R_1 \theta),$$
where the $R_j$ is the Riesz transform:
$$R_j(\theta)(x,t)={1 \over 2 \pi} PV \int_\RR^{2} {(x_j-y_j) \theta(y,t) \over |x-y|^{3}  } \dif y.$$
Therefore, the system $(\ref{QC1})-(\ref{QC3})$ reduces to
$$\theta_t + {\rm div} [ (R^{\perp} \theta) \theta ]=0.$$
One obtains the one-dimensional quasi-geostrophic equation by assuming that $\theta(x,t) \equiv \theta(x_1,t)$: integration of  the Riesz transform $R_2$ with respect to the variable $y_2$ results in a Hilbert transform of $\theta(x_1,t)$.

\medskip

The Hilbert transform is well characterized in terms of Fourier transform. Indeed, it can be equivalently defined
as
\[
\cF[H u](y)=-\ii \sgn(y) \cF[u](y)\,.
\]
%where
%\[
%\sigma(y) =
%\left\{
%\begin{array}{rr}
%1 & \mbox{if $y > 0$} \,, \\
%0 & \mbox{if $y=0$} \,, \\
%-1 & \mbox{if $y< 0$} \,.
%\end{array}
%\right.
%\]

The model $(\ref{eq:modelB})$ has been considered in the classical references \cite{CLM,DG,Schochet,MajdaB02}. In particular \cite{Mats} and \cite{BLM} consider the periodic case, and proof existence of finite-time blow-up $C^{\infty}(\TT \times [0,T))$-solutions for this equation.

The integral equation for this model, analogous to~\eqref{eq:integral:NS}, 
is given by
\begin{equation}\label{eq:integral:ModelB}
v(y,t) = \ee^{-|y|^\gamma t} v_0(y) + \int_0^t  \int_\RR y v(y-z,\tau) \sgn(y-z) v(z,\tau) 
\ee^{-|y|^\gamma (t-\tau)} \dif z\dif \tau\,.
\end{equation}
The Leray projection is  meaningless for $d=1$: it is identically equal to zero. The operator
\begin{equation}\label{eq:leray:d1}
  P_y v(z) = - \ii \sgn(y-z) v(z),
\end{equation}
appearing in $(\ref{eq:integral:ModelB})$ is, however, a projection. We will denote it by the same symbol $P_y$.

We will also consider the generalized version of $(\ref{eq:integral:NS})$:
\begin{equation}\label{eq:integral:NSgamma}
v(y,t) = \ee^{-|y|^\gamma t} v_0(y) + \ii \int_0^t \int_{\RR^d} (y \cdot v(y-z,\tau)) P_y v(z,\tau) \ee^{-|y|^\gamma (t-\tau)} \dif z \dif \tau\,, 
\end{equation}
for $\gamma>1$.

\subsection{The Cordoba-Cordoba-Fontelos equations}

Another interesting one-dimensional model is the model proposed in \cite{CCF}:
\begin{equation}\label{eq:CCF}
\pd_t u - H u \cdot u_x = \Lambda^\gamma u\,,
\end{equation}
where $Hu$ is given by~\eqref{eq:Hilbert}, and
$\Lambda^\gamma = (-\Delta)^{\gamma/2}$ is given in terms of the
fractional Laplacian. Let us recall that the fractional
Laplacian of order $s$ (in $\RR^d$, $d\geq 1$) is defined as
\begin{equation}\label{eq:FracDelta}
(-\Delta)^s u(x)=c_{d,s} \PV_{\RR^d}
\frac{u(x)-u(y)}{|x-y|^{d+2s}} \dif y\,,\qquad
c_{d,s} = \frac{4^s \Gamma(d/2+s)}{\pi^{d/2} |\Gamma(-s)|}\,,
\end{equation}
where $\Gamma$ is the Gamma function.
In the particular case $d=1$ and $s=1/2$, we have
\[
(-\Delta)^{1/2} u(x)=\frac{1}{\pi} \PV_{\RR} \frac{u(x)-u(y)}{(x-y)^{2}} \dif y
= \frac{1}{\pi} \PV_{\RR} \frac{u'(y)}{x-y} \dif y = H u'(x)\,.
\]
Moreover, for $d=1$, we have the property $H \Lambda^\gamma u = \pd_x \Lambda^{\gamma-1} u$.

The fractional Laplacian is well characterized in terms of
Fourier transform. Indeed, can be equivalently defined
as
\[
\cF[(-\Delta)^s u](y)=|y|^{2s} \cF[u](y).
\]

The integral equation for the model~\eqref{eq:CCF}, analogous to~\eqref{eq:integral:NS}, 
is given by
\begin{equation}\label{eq:integral:CCF}
v(y,t) = \ee^{-|y|^2 t} v_0(y) + \int_0^t \int_{-\infty}^\infty z v(y-z,\tau) \sgn(y-z) v(z,\tau) \dif z
\ee^{-|y|^2 (t-\tau)} \dif \tau\,.
\end{equation}
This integral equation is somewhat similar to $(\ref{eq:integral:ModelB})$, the significant difference is the multiplication by $z$ inside of the convulution term.

The following facts are known:
\begin{itemize}
\item For $\gamma>1$ the system~\eqref{eq:CCF} admits global existence of solutions (see ~\cite{CCF}).
\item For $\gamma=1$ and small data, the system~\eqref{eq:CCF} admits global existence of solutions (see ~\cite{CCF}).
\item For $\gamma=1$ and all data, the system~\eqref{eq:CCF} admits global existence of solutions (see in~\cite{Dong08}).
\item For $\gamma<1/2$, the system~\eqref{eq:CCF} has singular solutions (see ~\cite{LiR08}).
\item The problem is open for $1/2 \leq \gamma < 1$.
\end{itemize}

Presumably, the renormalization approach can be used to resolve the last case via a construction of {a-priori} bounds similar to the one given in this paper.

\subsection{A family of 1-dimensional model in hydrodynamics}
Let us consider the following family of PDEs:
\begin{equation}\label{eq:general1d}
\pd_t w +a (\Lambda^{-1}w) w_x- H w \cdot w = \Lambda^\gamma w\,,
\end{equation}
where $Hw$ is given by~\eqref{eq:Hilbert} and $\Lambda^{-1}=(-\Delta)^{-1/2}$ is given by~\eqref{eq:FracDelta}. This family consist in including a diffusion term in the parameter family considered in \cite{OkamotoSW} as a generalization of the models proposed in \cite{CCF,CLM,DG}. This continuum of models, in terms of the parameter $a$, give different ``weights'' to the vortex stretching and transport terms.

Here, $w$ should not be interpreted as the velocity $u$, but as the vorticity  $w=u_x$. The following facts are known:
\begin{itemize}
\item The case $\gamma=0$ and $a=0$ is in the so-called Constantin-Lax-Majda model \cite{CLM}. The authors of \cite{CLM} used special properties of $H$ to solve the equation exactly and  showed  existence of blow-up solutions $w$ such that the corresponding velocity remains bounded.
\item The case $\gamma=2$ and $a=0$, i.e. with dissipation $w_{xx}$,  was considered in ~\cite{Schochet}, which proves  existence of blow-up solutions $w$ such that the corresponding velocity also blows-up. This means that the Constantin-Lax-Majda model is is not a good hydrodynamics model in presence of diffusion. This is the reason why S. De Gregorio introduced a transport term $a=1$ in ~\cite{DG}.
\item The case $\gamma=0$ and $a=1$ is the De Grirorio model (see ~\cite{DG}).
\item The case $\gamma=0$ and $a=-1$ is the C\'ordoba-C\'ordoba-Fontelos model (cf. \cite{CCF}; simply take derivatives $\pd_x$ in \eqref{eq:CCF} and use the properties of $H$ and $\Lambda$). %According with my poor intuition, it seems that there is more chances of blow up in the vorticity model~\eqref{eq:general1d} with $a=-1$ than in \eqref{eq:CCF}.
\item The models in the case $\gamma=0$ and $a<0$ admits finite-time blow-up of smooth solutions (see ~\cite{Castro}).
\item The mode with  $\gamma=0$ and $a>0$, $a$- small, also has finite-time blow-ups (see ~\cite{EJ}).
\end{itemize}

The integral equation for this model, analogous to~\eqref{eq:integral:NS},  is given by
\begin{align}
\nonumber v(y,t) = \ee^{-y^2 t} v_0(y) &  - a \ii \int_0^t \int_{-\infty}^\infty z v(z,\tau) \frac{v(y-z,\tau)}{|y-z|} \ee^{-y^2 (t-\tau)} \dif z\dif \tau \\
 \label{eq:integral:general1d} & + \ii \int_0^t \int_{-\infty}^\infty \sgn(y-z) v(y-z,\tau) v(z,\tau) \ee^{-y^2 (t-\tau)} \dif z\dif \tau\,.
\end{align}

As it was mentioned above, if one takes $a=-1$, these integral equations are not the same as~\eqref{eq:integral:CCF}, since now $v$ is the Fourier transform of the vorticity $w=u_x$.


